A New Look and Convergence Rate of Federated Multi-Task Learning with Laplacian Regularization

Non-Independent and Identically Distributed (non- IID) data distribution among clients is considered as the key factor that degrades the performance of federated learning (FL). Several approaches to handle non-IID data such as personalized FL and federated multi-task learning (FMTL) are of great interest to research communities. In this work, first, we formulate the FMTL problem using Laplacian regularization to explicitly leverage the relationships among the models of clients for multi-task learning. Then, we introduce a new view of the FMTL problem, which in the first time shows that the formulated FMTL problem can be used for conventional FL and personalized FL. We also propose two algorithms FedU and dFedU to solve the formulated FMTL problem in communication-centralized and decentralized schemes, respectively. Theoretically, we prove that the convergence rates of both algorithms achieve linear speedup for strongly convex and sublinear speedup of order 1/2 for nonconvex objectives. Experimentally, we show that our algorithms outperform the algorithm FedAvg, FedProx, SCAFFOLD, and AFL in FL settings, MOCHA in FMTL settings, as well as pFedMe and Per-FedAvg in personalized FL settings.

==> experiments.tex <==
\section{Experiments}
\label{simulation}
%Trying with dataset in \cite{smith17NIPS}

In this section, we validate the performance of \OurAlg when the data  are heterogeneous and non-i.i.d in both strongly convex and nonconvex settings. We show vital advances of \OurAlg with Laplacian regularization in federated multi-task and personalized settings by comparing \OurAlg with cutting-edge learning algorithms including MOCHA, pFedMe, Per-FedAvg, and the vanilla FedAvg. The experimental results show that  \OurAlg achieves appreciable performance improvement over others in terms of testing accuracy.
%\hy{briefly describe the metric: test accuracy. There are many ways of measuring accuracy, is it the loss}

% The effect of other hyperparameters is presented in the supplementary document. %The experimental results show that our algorithm gains noticeable performance improvement from the vanilla FedAvg and  Per-FedAvg in terms of training loss convergence rate and test accuracy in various settings.

\subsection{Experimental Settings}
%The goals in this section are:
%\begin{itemize}
%	\item to identify the effect of hyperparameters such as $R$, $K$ and $\lambda$ to the convergence and performance of our algorithm;
%	\item to compare the performance, in terms of train loss and global accuracy, of our algorithm with those of FedAvg, Per-FedAvg and APFL; and
%	\item to compare the performances, in terms of test accuracy, of the algorithms above when using their best combination of hyperparameters.
%\end{itemize}
We consider classification problems using real datasets generated in federated settings, including  Human Activity Recognition, Vehicle sensor, MNIST, and CIFAR-10. %The full details on the datasets are provided as follow:
\begin{itemize}[noitemsep,nolistsep]
	\item  \textbf{Human Activity Recognition}: The set of data gathered from accelerometers and gyroscopes of cell phones from 30 individuals performing six different activities including lying-down, standing, walking, sitting, walking-upstairs, and walking-downstairs \cite{anguitaPublicDomainDataset2013}. Each individual is considered as a task (client) classifying 6 different activities.
	\item  \textbf{Vehicle Sensor}: Data is collected from a distributed wireless sensor network of 23 sensors including acoustic (microphone), seismic (geophone), and infrared (polarized IR sensor) \cite{duarteVehicleClassificationDistributed2004}. It aims to classify types of moving vehicles. We consider each sensor as a separate task (client) performing the binary classification to predict 2 vehicle types: Assault Amphibian Vehicle (AAV)  and Dragon Wagon (DW).
	\item \textbf{MNIST}:  A handwritten digit dataset \cite{lecunGradientbasedLearningApplied1998} includes 10 labels and 70,000 instances. The whole dataset is distributed  to $N = 100$ clients. Each client has a different local data size and consists of 2 over 10 labels.
	\item \textbf{CIFAR-10}:  An object recognition dataset \cite{krizhevskyLearningMultipleLayers} includes 60,000 colour images belonging to 10 classes. We partition the dataset to $N = 20$ clients and 3 labels per client.%\hy{is the partition done by you (not provided by the dataset)? then can briefly explain why N=20 and 3 labels...}
	\vspace{-0mm}
\end{itemize}

All datasets are split randomly with 75\% and 25\% for training and testing, respectively. %\hy{is the data splitting following the related work?} 
We use a multinomial logistic regression model (MLR) with cross-entropy loss functions and $L_2$-regularization term as the strongly convex model for Human Activity Recognition, Vehicle Sensor, and MNIST.  
%For nonconvex case, we use a simple DNN which has one hidden layer with ReLU activation function  for Human Activity Recognition, Vehicle Sensor and two hidden layers for MNIST. The size of hidden layers varying depends on the dataset.
For nonconvex setting, we apply a CNN network that has a similar structure to \cite{mcmahan17} for CIFAR-10 and a simple deep neural network (DNN) for other datasets. More details about datasets and the DNN structure are given in the supplementary material. 
%We follow the implementation of \cite{canh20NIPS} for pFedMe, Per-FedAvg and \cite{liangThinkLocallyAct2020} for MOCHA. 

It is noted that the structural dependence matrix $\Omega$ of MOCHA is chosen  as $\Omega = (\textbf{I}_{N \times N} - \frac{1}{N}\textbf{11}^T)^2$ in order to make the weight vectors close to their mean \cite{evgeniouRegularizedMultiTask2004}. As both \OurAlg and \dFed have the same performance when there is no client sampling, in our experiments, we only evaluate the performance of \OurAlg. During experiments, we assume that all clients have the same weight connection $a_{kl}$ with others. We also explain how we choose different values of $a_{kl}$ in the supplement. When comparing \OurAlg with other algorithms, we conduct 5-fold cross-validation to figure out the combination of hyperparameters allowing each algorithm to achieve the highest test accuracy.
%\hy{not clear: how a 5-fold cross validation tune hyperparamters for best accuracy? There are many systematic hyperparamter tunning methods (such as Grid search, BO, etc.)} 
The accuracy is reported with mean and standard deviation over 10 runs. All experiments were conducted using PyTorch \cite{paszkePyTorchImperativeStyle2019} version 1.6.%\hy{can also briefly say hardware settings}

\subsection{Performance of \OurAlg  in Federated Multi-Task Learning}
\label{sim:MTL}
\begin{table}[t!]
	\centering
	\caption{ Performance comparison of decentralized setting (All tasks participate, $R = 5$, $S=N$, mini-batch size $B = 20$, $\eta = 10^{-2}$, $T = 200$).}
	%, $\mu = 0.03$ for Human Activity, 0.02 for Vehical sensor}
	\begin{tabular}{l|l|ll}
		\multicolumn{1}{l|}{\multirow{2}{*}{Dataset} } & \multirow{2}{*}{Algorithm}  &  \multicolumn{2}{c}{Test accuracy}  \\ 
		&                                             & \multicolumn{1}{c}{Convex}        & \multicolumn{1}{c}{Nonconvex }   \\ \hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Human\\ Activity\end{tabular}}       
		& \OurAlg              &  $\textbf{99.10}      \pm 0.18$  &  $\textbf{99.21}      \pm 0.15$                   \\
		%& MOCHA         &          $ 98.97      \pm 0.04 $      &          $ 99.03      \pm 0.09 $                 \\
		& MOCHA         &          $ 98.79      \pm 0.04 $              \\
		& Local              &          $ 98.29    \pm 0.01$     &          $ 98.34    \pm 0.03$                \\
		& Global              		&  $93.79           		\pm 0.27$          &          $ 94.58    \pm 0.16$             \\ \hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Vehicle\\ Sensor\end{tabular}  }       
		& \OurAlg          &        $ \textbf{91.16}   \pm 0.02$                &        $ \textbf{95.43}   \pm 0.09$           \\
		& MOCHA         &    $     90.94      \pm 0.05$        &           \\
		& Local           &          $ 88.16    \pm 0.05 $          &          $ 92.10    \pm 0.06 $             \\
		& Global          &  $80.21  \pm 0.12 $            &  $83.00  \pm 0.11 $                \\ \hline
	\end{tabular}
	\label{T:compare_task}	
	\vspace{-4mm}
\end{table}
We first show the benefits of  \OurAlg in federated multi-task learning by comparing \OurAlg  with  Local model (training one separate model per client), Global model (training one single model on centralized data), and MOCHA, the conventional FMTL algorithm \cite{smith17NIPS}. Each client represents a separate task and all clients have the same weight connection $a_{kl}$ with others.  To compare with Local and Global models, both MOCHA and \OurAlg use full clients for training ($S= N$), and we only report the convex setting for MOCHA according to its assumption.
%We consider Human Activity, Vehicle Sensor, and MNIST datasets for multitask learning as the data among tasks are highly non-idd in natural but those data still have the connection. 

From the results in Table.~\ref{T:compare_task}, \OurAlg\ achieves the highest performance, followed by MOCHA, Local model, and Global model. The results are reasonable because both MOCHA and \OurAlg have the ability to learn models for multiple related tasks simultaneously and capture relationships amongst clients. Moreover, the Local model at individual client learns only its own data without any contribution from the model of other clients while the Global model only does a single task that is not well generalized on highly non-i.i.d  data. Therefore, \OurAlg is appropriate for handling the statistical difficulties in practical FL systems.
% Although the performance gap between \OurAlg  and MOCHA is slight in this experiment, MOCHA requires calculation on  matrix $W = [w_1 , ..., w_N]$ which is a matrix of all the weight vectors from $N$ clients. When the number of clients is large, MOCHA requires a significant computing resource compared to \OurAlg, which makes \OurAlg more practical than MOCHA in the FL system. 

%
%\begin{figure*}[htp]
%	\centering
%	\subfigure[random caption 1]{\includegraphics[scale=0.38]{Figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}\quad
%	\subfigure[random caption 2]{\includegraphics[scale=0.38]{Figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}
%\end{figure*}
\begin{figure*}[htp]
	\centering
	\vspace{-2mm}
	{\includegraphics[scale=0.323]{Figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/HUMAN_ACTIVITY_eta_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/HUMAN_ACTIVITY_eta_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/HUMAN_ACTIVITY_eta_train_non_convex.pdf}}
	\vspace{-2mm}
	\caption{Effects of $\eta$ for both strongly convex and nonconvex settings on Human Activity with cut-off data.}
	\label{F:Human_eta}	
\end{figure*}
\begin{figure*}[htp]
	\centering
	\vspace{-2mm}
	{\includegraphics[scale=0.323]{Figs/VEHICLE_SENSOR_eta_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/VEHICLE_SENSOR_eta_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/VEHICLE_SENSOR_eta_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{Figs/VEHICLE_SENSOR_eta_train_non_convex.pdf}}
	\vspace{-2mm}
	\caption{Effects of $\eta$  for both strongly convex and nonconvex settings on Vehicle Sensor with cut-off data.}
	\label{F:Vehicle_eta}	
	\vspace{-3mm}
\end{figure*}
\subsection{Advantages of Laplacian Regularization in Multi-Task Learning}
In practical FL networks, some clients have significantly limited data sizes and need collaborative learning with others. We hence randomly cut off around 90\% local data of more than a half of the total clients to observe the behavior of \OurAlg, MOCHA, Local model, and Global model, and how Laplacian regularization affects \OurAlg in this scenario. \\
We evaluate  \OurAlg  on a wide range of values of $\eta \in \{10^{-3},10^{-2},10^{-1}, 1\}$. The experimental results in Figs.~\ref{F:Human_eta} and~\ref{F:Vehicle_eta} show that \OurAlg  appreciably outperforms the others. Thanks to Laplacian regularization, \OurAlg utilizes additional information about the structures of clients' model to increase the learning performance, and the contribution from clients having the large data size to those having smaller one becomes more significant. The larger $\eta$ is, the more the contributions from other clients are. However, when $\eta$ reaches a certain threshold, it has a considerably negative impact on the performance of \OurAlg. %With a given value of $a_{kl}$ or $\rho$, $\eta$ should be not too large to satisfy the condition $\eta\rho > 2\beta$, which has been mentioned above in the theoretical analysis. 
These results further show that \OurAlg is appropriate for few-shot learning where clients having limited samples are able to learn from the prior knowledge of clients having more data samples.\\ We also recognize that Local model suffers overfitting when the data size at clients is small. While the training loss of Local model is small,  its test accuracy is extremely lower than others in all settings. By contrast, the performance of the Global model
is only negligibly affected in this scenario. Additionally,  MOCHA shows the worse performance in the case of Human Activity dataset in Fig.~\ref{F:Human_eta}. This 
 may be due to the structural dependence matrix $\Omega$ that is not as robust as the structure of Laplacian regularization.  
\subsection{Comparison with Personalized FL algorithms}
Finally, we compare \OurAlg with not only MOCHA and FedAvg but also the state-of-the-art personalized FL algorithms such as pFedMe and Per-FedAvg  in Table.~\ref{T:compare_performance}.
%\hy{Furthermore, we compare \OurAlg with the state-of-the-art personalized FL algorithms such as pFedMe and Per-FedAvg  in Table.~\ref{T:compare_performance}.}
In this experiment, we fix the subset of clients $S = 0.1 N$ and perform the comparison on two datasets MNIST and CIFAR-10. We also conduct additional comparisons on Human Activity and Vehicle Sensor datasets, which are presented in the supplement. Overall,  \OurAlg\ maintains the top performance in all scenarios, followed by pFedMe, Per-FedAvg, and FedAvg. Both MOCHA and \OurAlg have a similar performance in the case of MNIST. The performance improvement of \OurAlg compared to the conventional FL and personalized FL algorithms mainly comes from the advance of additional information about the relationships of clients' models which are captured by the entity graph but not in the star graph (as discussed in Section~\ref{sec:unifiedproblem}). 
%All clients’ models in \OurAlg not only have relationships with their neighboring clients. 
%\textcolor[rgb]{0.00,0.00,1.00}{(explain more star graph)}
\begin{table}[t!]
	\centering
	\caption{ Performance comparison of centralized setting ($R = 5$, $ S = 0.1 N$, $B = 20$, $T = 200$). MNIST uses MLR model while CIFAR uses CNN model.}
	\begin{tabular}{l|ll}
		\multirow{2}{*}{Algorithm}  &   \multicolumn{2}{c}{Test accuracy} \\ 
		& \multicolumn{1}{c}{MNIST}        & \multicolumn{1}{c}{CIFAR-10}   \\ \hline
		\OurAlg                  & $ \textbf{97.82}      \pm 0.02$    &     $\textbf{79.40}    \pm 0.25 $                        \\
		MOCHA      &       $ 97.80 \pm 0.02  $          \\	
		pFedMe             &          $ 95.38    \pm 0.09$         &    $    78.70 \pm 0.15 $               \\
		Per-FedAvg               &       $ 91.77     \pm 0.23  $       &           $67.61     \pm 0.03 $                      \\
		FedAvg            		&  $90.14         		\pm 0.61$    &           $36.32     \pm 5.57 $                       \\ \hline
	\end{tabular}
	\label{T:compare_performance}	
	\vspace{-2mm}
\end{table}



==> experiments_arxiv.tex <==
\section{Experiments}
\label{simulation}
%Trying with dataset in \cite{smith17NIPS}

In this section, we validate the performance of \OurAlg when the data are heterogeneous and non-i.i.d in both strongly convex and nonconvex settings. We show vital advances of \OurAlg with Laplacian regularization in federated multi-task and personalized settings by comparing \OurAlg with cutting-edge learning algorithms including MOCHA, pFedMe, Per-FedAvg, and the vanilla FedAvg. The experimental results show that  \OurAlg achieves appreciable performance improvement over others in terms of testing accuracy.

\subsection{Experimental Settings}
We consider classification problems using real datasets generated in federated settings, including  Human Activity Recognition, Vehicle sensor, MNIST, and CIFAR-10. %The full details on the datasets are provided as follow:
\begin{itemize}[noitemsep,nolistsep]
	\item  \textbf{Human Activity Recognition}: The set of data gathered from accelerometers and gyroscopes of cell phones from 30 individuals performing six different activities including lying-down, standing, walking, sitting, walking-upstairs, and walking-downstairs \cite{anguitaPublicDomainDataset2013}. Each individual is considered as a task (client) classifying 6 different activities.
	\item  \textbf{Vehicle Sensor}: Data is collected from a distributed wireless sensor network of 23 sensors including acoustic (microphone), seismic (geophone), and infrared (polarized IR sensor) \cite{duarteVehicleClassificationDistributed2004}. It aims to classify types of moving vehicles. We consider each sensor as a separate task (client) performing the binary classification to predict 2 vehicle types: Assault Amphibian Vehicle (AAV)  and Dragon Wagon (DW).
	\item \textbf{MNIST}:  A handwritten digit dataset \cite{lecunGradientbasedLearningApplied1998} includes 10 labels and 70,000 instances. The whole dataset is distributed  to $N = 100$ clients. Each client has a different local data size and consists of 2 over 10 labels.
	\item \textbf{CIFAR-10}:  An object recognition dataset \cite{krizhevskyLearningMultipleLayers} includes 60,000 colour images belonging to 10 classes. We partition the dataset to $N = 20$ clients and 3 labels per client.%\hy{is the partition done by you (not provided by the dataset)? then can briefly explain why N=20 and 3 labels...}
	\vspace{-0mm}
\end{itemize}

In practical FL networks, some clients have significantly limited data sizes and need collaborative learning with others. For each dataset, we hence down-sample 80 \% data belong to half of the total clients to observe behaviour of all clients. The result without down--sampling is provided in Appendix. All datasets are split randomly with 75\% and 25\% for training and testing, respectively. %\hy{is the data splitting following the related work?} 

We use a multinomial logistic regression model (MLR) with cross-entropy loss functions and $L_2$-regularization term as the strongly convex model for Human Activity Recognition, Vehicle Sensor, and MNIST.  
%For nonconvex case, we use a simple DNN which has one hidden layer with ReLU activation function  for Human Activity Recognition, Vehicle Sensor and two hidden layers for MNIST. The size of hidden layers varying depends on the dataset.
For nonconvex setting, we use  a simple deep neural network (DNN) with one hidden layer, a ReLU activation function, and a softmax layer at the end of the network for Human Activity and Vehicle Sensor datasets. The size of hidden layer is 100 for Human Activity and 20 for Vehicle Sensor. In the case of MNIST, we use DNN with 2 hidden layers and both layers have the same size of 100.  For CIFAR-10, we follow the CNN structure of \cite{mcmahan17}. 
%We follow the implementation of \cite{canh20NIPS} for pFedMe, Per-FedAvg and \cite{liangThinkLocallyAct2020} for MOCHA. 

The structural dependence matrix $\Omega$ of MOCHA is chosen  as $\Omega = (\textbf{I}_{N \times N} - \frac{1}{N}\textbf{11}^T)^2$, where $\textbf{I}_{N \times N}$ is the identity matrix with size $N \times N$ and $\textbf{1}$ is a vector of all ones size $N$, in order to make the weight vectors close to their mean \cite{evgeniouRegularizedMultiTask2004}. As both \OurAlg and \dFed have the same performance when there is no client sampling, in our experiments, we only evaluate the performance of \OurAlg.  When comparing \OurAlg with other algorithms, we conduct 5-fold cross-validation to figure out the combination of hyperparameters allowing each algorithm to achieve the highest test accuracy.
%\hy{not clear: how a 5-fold cross validation tune hyperparamters for best accuracy? There are many systematic hyperparamter tunning methods (such as Grid search, BO, etc.)} 
All experiments are implemented using PyTorch \cite{paszkePyTorchImperativeStyle2019} version 1.6. We follow the implementations  of \cite{canh20NIPS} for pFedMe, FedAvg, and Per-FedAvg, \cite{liangThinkLocallyAct2020} for MOCHA. All  experiments are run on \textbf{NVIDIA Tesla T4} GPU. Each experiment is run 10 times for statistical reports. All code and data are published at \footnote{\url{https://github.com/dual-grp/FedU_FMTL}}. The accuracy is reported with mean and standard deviation over 10 runs. 
\subsection{Performance of \OurAlg  in Federated Multi-Task Learning}
\label{sim:MTL}
\begin{figure*}[t!]
	\centering
	%	\vspace{-2mm}
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_eta_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_eta_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_eta_train_non_convex.pdf}}
	%\vspace{-2mm}
	\caption{Effects of $\eta$ for both strongly convex and nonconvex settings on Human Activity with cut-off data.}
	\label{F:Human_eta}	
\end{figure*}
\begin{figure*}[t!]
	\centering
	%\vspace{-2mm}
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_eta_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_eta_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_eta_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_eta_train_non_convex.pdf}}
	%\vspace{-2mm}
	\caption{Effects of $\eta$  for both strongly convex and nonconvex settings on Vehicle Sensor with cut-off data.}
	\label{F:Vehicle_eta}	
	%\vspace{-3mm}
\end{figure*}

\begin{figure*}[t!]
	\centering
	%	\vspace{-3mm}
	{\includegraphics[scale=0.323]{figs/MNIST_eta_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/MNIST_eta_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/MNIST_eta_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/MNIST_eta_train_non_convex.pdf}}
	%	\vspace{-3mm}
	\caption{Effects of $\eta$ for both strongly convex and nonconvex settings  on MNIST with cut-off data.}
	\label{F:Mnist_eta}	
\end{figure*}
\begin{figure*}[t!]
	\centering
	\vspace{-3mm}
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_akl_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_akl_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_akl_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/HUMAN_ACTIVITY_akl_train_non_convex.pdf}}
	\vspace{-3mm}
	\caption{Effects of $\{a_{kl}\}$  for both strongly convex and nonconvex settings on Human Activity with cut-off data.}
	\label{F:Human_akl}	
\end{figure*}
\begin{figure*}[t!]
	\centering
	\vspace{-3mm}
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_akl_test_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_akl_train_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_akl_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.323]{figs/VEHICLE_SENSOR_akl_train_non_convex.pdf}}
	\vspace{-3mm}
	\caption{Effects of $\{a_{kl}\}$  for both strongly convex and nonconvex settings  on Vehicle Sensor with cut-off data.}
	\label{F:Vehicle_akl}	
\end{figure*}

\begin{figure*}[t!]
	\centering
	\vspace{-3mm}
	{\includegraphics[scale=0.32]{figs/MNIST_akl_test_convex.pdf}}\quad
	{\includegraphics[scale=0.32]{figs/MNIST_akl_train_convex.pdf}}\quad
	{\includegraphics[scale=0.32]{figs/MNIST_akl_test_non_convex.pdf}}\quad
	{\includegraphics[scale=0.32]{figs/MNIST_akl_train_non_convex.pdf}}
	\vspace{-3mm}
	\caption{Effects of $\{a_{kl}\}$ for both strongly convex and nonconvex settings  on MNIST with cut-off data.}
	\label{F:Mnist_akl}		
\end{figure*}
We first show the benefits of  \OurAlg in federated multi-task learning by comparing \OurAlg  with  Local model (training one separate model per client), Global model (training one single model on centralized data), and MOCHA, the conventional FMTL algorithm \cite{smith17NIPS}. Each client represents a separate task and all clients have the same weight connection $\{a_{kl}\}$  with others.  To compare with Local and Global models, both MOCHA and \OurAlg use full clients for training ($S= N$), and we only report the convex setting for MOCHA according to its assumption.
%We consider Human Activity, Vehicle Sensor, and MNIST datasets for multitask learning as the data among tasks are highly non-idd in natural but those data still have the connection. 


From the results in Table.~\ref{T:compare_task}, \OurAlg\ achieves the highest performance, followed by MOCHA, Local model, and Global model. The results are reasonable because both MOCHA and \OurAlg have the ability to learn models for multiple related tasks simultaneously and capture relationships amongst clients. Moreover, the Local model at individual client learns only its own data without any contribution from the model of other clients while the Global model only does a single task that is not well generalized on highly non-i.i.d  data. Therefore, \OurAlg is appropriate for handling the statistical difficulties in practical FL systems.
% Although the performance gap between \OurAlg  and MOCHA is slight in this experiment, MOCHA requires calculation on  matrix $W = [w_1 , ..., w_N]$ which is a matrix of all the weight vectors from $N$ clients. When the number of clients is large, MOCHA requires a significant computing resource compared to \OurAlg, which makes \OurAlg more practical than MOCHA in the FL system. 

%
%\begin{figure*}[htp]
%	\centering
%	\subfigure[random caption 1]{\includegraphics[scale=0.38]{Figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}\quad
%	\subfigure[random caption 2]{\includegraphics[scale=0.38]{Figs/HUMAN_ACTIVITY_eta_test_convex.pdf}}
%\end{figure*}


\subsection{Advantages of Laplacian Regularization in Multi-Task Learning}
% In practical FL networks, some clients have significantly limited data sizes and need collaborative learning with others. We hence randomly cut off around 90\% local data of more than a half of the total clients to observe the behavior of \OurAlg, MOCHA, Local model, and Global model, and how Laplacian regularization affects \OurAlg in this scenario. \\
We evaluate  \OurAlg  on a wide range of values of $\eta \in \{10^{-3},10^{-2},10^{-1}, 1\}$. The experimental results in Figs.~\ref{F:Human_eta} and~\ref{F:Vehicle_eta} show that \OurAlg  appreciably outperforms the others. Thanks to Laplacian regularization, \OurAlg utilizes additional information about the structures of clients' model to increase the learning performance, and the contribution from clients having the large data size to those having smaller one becomes more significant. The larger $\eta$ is, the more the contributions from other clients are. However, when $\eta$ reaches a certain threshold, it has a considerably negative impact on the performance of \OurAlg. %With a given value of $a_{kl}$ or $\rho$, $\eta$ should be not too large to satisfy the condition $\eta\rho > 2\beta$, which has been mentioned above in the theoretical analysis. 
These results further show that \OurAlg is appropriate for few-shot learning where clients having limited samples are able to learn from the prior knowledge of clients having more data samples.\\ We also recognize that Local model suffers overfitting when the data size at clients is small. While the training loss of Local model is small,  its test accuracy is extremely lower than others in all settings. By contrast, the performance of the Global model
is only negligibly affected in this scenario. Additionally,  MOCHA shows the worse performance in the case of Human Activity dataset in Fig.~\ref{F:Human_eta}. This 
 may be due to the structural dependence matrix $\Omega$ that is not as robust as the structure of Laplacian regularization.  
% \begin{table}[t!]
% 	\centering
% 	\caption{ Performance comparison of centralized setting ($R = 5$, $ S = 0.1 N$, $B = 20$, $T = 200$). MNIST uses MLR model while CIFAR uses CNN model.}
% 	\begin{tabular}{l|ll}
% 		\multirow{2}{*}{Algorithm}  &   \multicolumn{2}{c}{Test accuracy} \\ 
% 		& \multicolumn{1}{c}{MNIST}        & \multicolumn{1}{c}{CIFAR-10}   \\ \hline
% 		\OurAlg                  & $ \textbf{97.82}      \pm 0.02$    &     $\textbf{79.40}    \pm 0.25 $                        \\
% 		MOCHA      &       $ 97.80 \pm 0.02  $          \\	
% 		pFedMe             &          $ 95.38    \pm 0.09$         &    $    78.70 \pm 0.15 $               \\
% 		Per-FedAvg               &       $ 91.77     \pm 0.23  $       &           $67.61     \pm 0.03 $                      \\
% 		FedAvg            		&  $90.14         		\pm 0.61$    &           $36.32     \pm 5.57 $                       \\ \hline
% 	\end{tabular}
% 	\label{T:compare_performance}	
% 	\vspace{-2mm}
% \end{table}

\subsection{Effect of the Graph Information $\{a_{kl}\}$} 
For the above experiments, we assume that all relationships among a client and its neighbors are equal. However, in practice, the connection weights may have different values and they need to be known in advance. In this session, we evaluate the effect of graph information on three datasets including Human Activity, Vehicle Sensor, and MNIST with the cut-off data setting. We normalize the values of $\{a_{kl}\}$in the range of  $[0, 1]$.  In this section, we simulate 4 different scenarios of $\{a_{kl}\}$ as below: 
\begin{itemize}
	\item Random (R): All values of $\{a_{kl}\}$ are generated radomly $\{a_{kl}\} \thicksim \mathcal{N}(0, 1)$.
	\item Equal (E):  All $\{a_{kl}\}$ have a same value. We note that when all clients have the same value for $\{a_{kl}\}$, we can choose any value of $\{a_{kl}\}$ in the range of  $[0, 1]$. However, there will be one value of $\eta* \{a_{kl} \}$ allows \OurAlg to achieve the highest accuracy. So, whenever  $\{a_{kl}\}$  is large, we can choose a small $\eta$, and vice versa. In this experiment, we fix $\{a_{kl}\}$ and adjust $\eta$ accordingly. 
	
	\item Weighted (W): In the cutting-off data setting, there are various clients having significantly small data sizes. We set $\{a_{kl}\} = 0$ on the connection between these clients. We then set $\{a_{kl}\} = 0.5$ on the connection among clients having small data sizes and those having large data sizes, and  $\{a_{kl}\} = 1$ for all other connections.
	
	\item Similar (S): This scenario is only for MNIST. When distributing data to all clients, each client has 2 labels over 10.  Hence, clients may share only one, two similar labels or none of them. We set $\{a_{kl}\} = 0$, $\{a_{kl}\} = 0.5$, and $\{a_{kl}\} = 1$  for the connections among clients having no similar label, one similar label, and two similar labels, respectively.		
\end{itemize}

For all datasets, the performance of \OurAlg when $\{a_{kl}\}$ are weighted is better than that when all  $\{a_{kl}\}$ are equal. Especially for MNIST, when  $\{a_{kl}\}$ are weighted based on the similarity of clients, \OurAlg achieves the highest performance compared to other scenarios.  When $\{a_{kl}\}$ are generated randomly, the performance of \OurAlg is unpredictable; however, in most of the cases, the performance of \OurAlg with random $\{a_{kl}\}$ is better than that with equal $\{a_{kl}\}$. %So, the weight connection $a_{kl}$ plays a vital role in the performance behavior of \OurAlg. 

\subsection{Comparison with Personalized FL algorithms}
Finally, we compare \OurAlg with not only MOCHA and FedAvg but also the state-of-the-art personalized FL algorithms such as pFedMe and Per-FedAvg  in Table.~\ref{T:compare_performance}.
%\hy{Furthermore, we compare \OurAlg with the state-of-the-art personalized FL algorithms such as pFedMe and Per-FedAvg  in Table.~\ref{T:compare_performance}.}
In this experiment, we fix the subset of clients $S = 0.1 N$ and perform the comparison on all four real datasets. Overall, that \OurAlg almost maintains the top performance in all scenarios. Only in the nonconvex case on MNIST, pFedMe performs slightly better than \OurAlg. The performance improvement of \OurAlg compared to the conventional FL and personalized FL algorithms mainly comes from the advance of additional information about the relationships of clients' models which are captured by the entity graph but not in the star graph (as discussed in Section~\ref{sec:unifiedproblem}). 
%All clients’ models in \OurAlg not only have relationships with their neighboring clients. 
%\textcolor[rgb]{0.00,0.00,1.00}{(explain more star graph)}


\begin{table}[t!]
	\centering
	\caption{ Performance comparison of centralized setting ($R = 5$, $ S = 0.1 N$, $B = 20$, $T = 200$).}
	%	\begin{tabular}{l|l|ll}
	\begin{tabular}{l|c|ll}
		\multirow{3}{*}{Dataset} & \multirow{3}{*}{Algorithm} & \multicolumn{2}{c}{Test Accurancy}                                                                                        \\
		&                            & \multicolumn{1}{c}{Convex} & \multicolumn{1}{c}{Non Convex} \\ \hline
		\multirow{4}{*}{CIFAR-10 }      
		& \OurAlg      &                &     $\textbf{79.40}    \pm 0.25 $                       \\
		%& MOCHA      &                 &    $  79.25         \pm 0.01 $                     \\
		& pFedMe    &             &    $    78.70 \pm 0.15 $                            \\
		& Per-FedAvg        &           &           $67.61     \pm 0.03 $                                   \\ 
		& FedAvg        &           		&  $36.32          		\pm 5.57$                     \\ \hline
		\multirow{4}{*}{MNIST}      
		& \OurAlg                  & $ \textbf{97.82}      \pm 0.02$                & $ 98.44     \pm 0.02$        \\
		%	& MOCHA      &       $ 97.80 \pm 0.02  $          &          $    97.86 \pm 0.02  $              &       $ 96.18 \pm 0.09  $               \\	
		& MOCHA      &       $ 97.80 \pm 0.02  $               \\	
		& pFedMe             &          $ 95.38    \pm 0.09$            &$\textbf{99.04} \pm 0.02$      \\
		& Per-FedAvg               &       $ 91.77     \pm 0.23  $ &       $ 97.59     \pm 0.30  $                \\
		& FedAvg            		&  $90.14         		\pm 0.61$     	&  $90.74         		\pm 1.62$                  \\ \hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Vehicle\\ Sensor\end{tabular}  }       
		& \OurAlg             &        $ \textbf{89.84}   \pm 0.06$     &        $ \textbf{94.18}   \pm 0.08$          \\
		%& MOCHA      &    $  89.73  \pm 0.89 $            &    $     90.63      \pm 0.16$              &    $  87.31  \pm 0.23 $        	 \\
		& MOCHA      &    $  89.73  \pm 0.89 $              	 \\
		& pFedMe         &            $85.87 \pm 0.02$                 &            $92.23 \pm 0.17$   		\\
		& Per-FedAvg           &         $82.21 \pm 0.01$    &         $87.50 \pm 1.21$               \\
		& FedAvg          &  $81.54  \pm 0.03 $    &  $85.61  \pm 0.07 $           \\ \hline
		\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} Human\\ Activity\end{tabular}}       
		%& \OurAlg      &     $0.03$               &  $\textbf{97.75}      \pm 0.21$                   	 \\
		& \OurAlg               &  $\textbf{97.75}      \pm 0.21$   &  $ \textbf{97.85}      \pm 0.39$      	 \\
		%& MOCHA      &       $ 97.69    \pm 0.03 $          &          $ 97.80      \pm 0.01 $         &          $ 92.33      \pm 0.67 $              	\\
		& MOCHA      &       $ 97.69    \pm 0.03 $               	\\
		& pFedMe             &          $ 97.52      \pm 0.09$         &          $ 97.60      \pm 0.09$             		\\
		& Per-FedAvg              &       $ 96.04      \pm 0.36  $    &       $ 96.21      \pm 0.33  $               \\
		& FedAvg             		&  $95.58           		\pm 0.05$  	&  $94.84           		\pm 0.07$           \\ \hline
	\end{tabular}
	\label{T:compare_performance}	
\end{table}

==> summary_change.tex <==
The reviewers have found merits in this manuscript. But as pointed out by the reviewers, the authors are advised to make a further discussion on the communication burden of dFedU, and provide a more comprehensive experiment comparison.

\textbf{Reviewer: 1}
\begin{enumerate}
	\item The paper mentions that there are usually relationships between the models of the clients and whether the proposed method can be extracted from the similar relationships between the clients by visualization methods or other methods in the experimental results.
	\item Does the relationship between the clients become irreversible, i.e., the adjacency matrix may be asymmetric?
	\item The Algorithm dFedU also creates a communication burden when a large number of clients exist, because the client needs to communicate with the rest of the large number of clients.
	\item What effect does the degree of Non-IID have on the model? Please provide experiments for analysis. There are many algorithms that improve on the traditional FL, please compare with it? (e.g. FedProx, AFL, SCAFFOLD, )
	\item The experimental results in Figure 3 are compared with MOCHA only, what about other comparison methods?
\end{enumerate}

\textbf{Reviewer: 2}
\begin{enumerate}
	\item Comments to the Author
	The paper proposed a decentralized federated learning and show that the conventional server-client federated learning is one of its special case. The paper is very well-written, and the experiment well demonstrate the optimality of the proposed algorithm. My only comment is that the proof should be given with the submitted manuscript, not put apart at the arxiv site. 
	
\end{enumerate}

\textbf{Reviewer: 3}
Comments to the Author
This paper takes weighted relationship among clients as a priori in federated multi-task learning. Two algorithms are respectively proposed for communication-centralized and decentralized schemes. They are proved to achieve good convergence rate. Furthermore, the authors prove several existing federated learning methods are all special cases of the proposed method. Experiments on four databases for different tasks show the method’s benefits. Different ways to decide priori relationship among clients are also provided for comparison.
The paper is easy to read and follow besides the formula derivation parts. For federated learning, especially when non-IID data distributions exist, relationships among clients are valuable, and it is well motivated in this paper. The method is not only proposed for strongly convex cases and communication-centralized schemes, but also for nonconvex cases and decentralized schemes. Adequate experiments are conducted and the results seem quite impressive. 
However, I have some concerns. 

\begin{enumerate}
	\item      In Figure 2, the role of the squares and circles are not clearly explained. And what is “true opt.”? 
	\item     The experimental section is mainly occupied by figures, which are suggested to present more tables recording the final results. 
	\item      The proposed method requires multiple steps for model updating on all clients, which is hard to achieve in some practical applications. This should be discussed.
	\item   So many (around 20) arXiv papers are cited. Better cite more peer-reviewed papers of top journals and conferences.
\end{enumerate}






